Relevant HAL Interface Requirements for Embedded Systems

Embedded applications often use a Hardware Abstraction Layer (HAL) to access hardware. Improper use of the HAL can lead to incorrect hardware operations, resulting in system failure and potentially serious damage to the hardware. The question is how one can obtain prioritize, among a possibly large set of HAL interface requirements, those that are indisputably relevant for preventing this kind of system failure. In this paper, we introduce a formal notion of relevance. This allows us to leverage a formal method, i.e., software model checking, to produce a mathematical proof that a requirement is indisputably relevant. We propose an approach to extract provably relevant requirements from issue reports on system failures. We present a case study to demonstrate that the approach is feasible in principle. The case study uses three examples of issue reports on embedded applications that use the SPI bus via the spidev HAL. The overall contribution of this paper is to pave the way for the study of approaches to a new kind of prioritization aimed at preventing a specific kind of system failure.

==> modes.tex <==
% !TeX spellcheck = en_US

% patch internal macros to obtain valid metadata for PDF file
\makeatletter
  \ifdef{\pdfmetadata}{
    \let\thetitle\@pdftitle
    \let\theauthor\@author
    \let\thepdfauthor\@pdfauthor
    \let\thepdfkeywords\@pdfkeywords
    \let\thedate\@date
  }{}
\makeatother

% patch internal macros to obtain valid DOI for the watermark
\makeatletter
  \ifdef{\watermark}{
    \let\thedoipublished\@doipublished
  }{}
\makeatother

% include package to set PDF specific data (color links, set metadata)
\ifdef{\pdfmetadata}{
  \usepackage[
    colorlinks,
    pdfencoding=auto,
    bookmarks
  ]{hyperref}
  \hypersetup{
    pdftitle={\thetitle},
    pdfauthor={\thepdfauthor},
    pdfkeywords={\thepdfkeywords},
    colorlinks=false,
    pdfborderstyle={/S/U/W 1},
    pdfborder=0 0 1
  }
  % package for printing the ORCiD logo
  \usepackage{orcidlink}
  \renewcommand{\orcidID}[1]{\orcidlink{#1}}
}{
  % ingore ORCiD from the authors
  %\renewcommand{\orcidID}[1]{}
}

% package to reference labels in text
\usepackage{cleveref}

% include package to print author's version watermark
\ifdef{\watermark}{
  \usepackage[
    angle=90,
    hpos=1in
  ]{draftwatermark}
  \SetWatermarkFontSize{25pt}
  \SetWatermarkScale{1.25}
  \SetWatermarkText{%
    {Pre-published (Author's) Version}
    \ifx\thedoipublished\empty\else
      \\{\small Published version is available at: \url{https://doi.org/\thedoipublished}}
    \fi
  }
}{}

% include package to show line numbers in draft mode
\ifdef{\draftmode}{
  \usepackage[
    switch
  ]{lineno}
  \linenumbers
}{}


==> vars.tex <==
% !TeX spellcheck = en_US

\makeatletter
% define macros to set PDF metadata
\def\pdftitle#1{\gdef\@pdftitle{#1}}
\def\@pdftitle{\@latex@warning@no@line{No \noexpand\pdftitle given}}
\def\pdfauthor#1{\gdef\@pdfauthor{#1}}
\def\@pdfauthor{\@latex@warning@no@line{No \noexpand\pdfauthor given}}
\def\pdfkeywords#1{\gdef\@pdfkeywords{#1}}
\def\@pdfkeywords{\@latex@warning@no@line{No \noexpand\pdfkeywords given}}
% define macro to set DOI of published paper in watermark text
\def\doipublished#1{\gdef\@doipublished{#1}}
\def\@doipublished{}
\makeatother

